Relative Langlands Duality

We propose a duality in the relative Langlands program. This duality pairs a Hamiltonian space for a group $G$ with a Hamiltonian space under its dual group $\check{G}$, and recovers at a numerical level the relationship between a period on $G$ and an $L$-function attached to $\check{G}$; it is an arithmetic analog of the electric-magnetic duality of boundary conditions in four-dimensional supersymmetric Yang-Mills theory.

==> local-geometric1.tex <==
 
\newcommand{\GX}{\mathsf{GX}}
\newcommand{\std}{\mathrm{std}}
 
\section{Unramified local  duality} 
\label{section-unramified-local}

 



 

\subsubsection{Setup}  \label{uld setup}

Let $\FF$ be either the complex numbers $\C$ or the algebraic closure $\overline{\mathbb{F}_q}$ of a finite field. In this section we will work with a dual pair as in \S \ref{goodhypersphericalpairs}:
$(G, M)$ will be a split hyperspherical pair defined over $\FF$,
for which $M$ admits a distinguished polarization  $M = T^*(X,\Psi)$,
and $(\check{G}, \check{M})$ its dual defined over $\kk$;
this coefficient field $\kk$ will be almost always be taken to be $\C$ or the algebraic closure of an $\ell$-adic field
according to whether $\FF$ is $\C$ or of finite characteristic. 

Occasionally, we will implicitly assume that everything is defined over $\mathbb F_q$, and will introduce Weil structures that the reader can ignore over the algebraic closure. In particular, the appearance of $k\langle 1\rangle:= k[1](\frac{1}{2})$ suggests that we have chosen a square root of the cyclotomic twist, and the twist by $(\frac{1}{2})$ can be ignored by readers interested in statements over $\C$ or $\overline{\mathbb F_q}$. 



As in \S \ref{localfieldnotn}, 
let $F = \FF((t))$, with integer ring $O = \FF[[t]]$. As before, when $\FF = \overline{\FF_q}$, we will be using $\ff, \fo$ to denote $\FF_q((t))$, $\FF_q[[t]]$. We will be using $X_O$ for the formal arc space, representing the functor $R\mapsto X(R[[t]])$, and $X_F$ for the formal loop space, representing $R\mapsto X(R((t)))$.
For $X$ affine, these are schemes and ind-schemes respectively. 


\subsubsection{} 
In this part we introduce and study the local conjecture, Conjecture~\ref{local conjecture}, a counterpart of the geometric Satake correspondence for spherical varieties. The conjecture asserts an equivalence
$$\boxed{
\SHV(X_F/G_O)\simeq \QCshear(\Mv/\Gv)
}$$
between the categories of $G_O$-equivariant sheaves on $X_F$ and $\Gv$-equivariant quasicoherent sheaves on $\Mv$,
but with the latter category {\em sheared} (i.e., cohomologically regraded) using the $\GGm$-action on $\Mv$. We also state a version for ``small'' categories, matching constructible sheaves and perfect complexes. The equivalence is required to respect various structures on the two sides:
\begin{itemize}
\item[$\bullet$] the basic object (structure sheaf of the arc space $X_O$) is taken to the structure sheaf of $\Mv$ (\S\ref{pointings});
\item[$\bullet$] the Hecke action on $X_F/G_O$ is matched (under derived Satake) with the moment map $\Mv/\Gv\to \fgxv/\Gv$ (\S\ref{Hecke local conj});
\item[$\bullet$] the action of Frobenius on $X_F$ is matched with the action of the grading group $\GGm$ on $\Mv$ (\S \ref{Galois local conj}); and
\item[$\bullet$] the loop rotation structure on $X_F$ is matched with the Poisson structure on $\Mv$ (\S\ref{Poisson local conj},  \S \ref{Poisson from loop}).
\end{itemize}


Some significant aspects of the conjecture are discussed elsewhere. We defer to \S \ref{PlancherelCoulomb} the discussion of the various aspects of the local conjecture which are most concretely understood in terms of the Plancherel algebra (or relative Coulomb branch), a ring object in the spherical Hecke category. 
 In \S \ref{automorphic-factorization} and \S \ref{spectral-factorization} we discuss a crucial additional structure on the local conjecture, namely compatibility with {\em factorization structures} on the two sides (and the action of changes of coordinates) as well as with the global conjecture. 
  
 \begin{itemize}
 \item In \S \ref{spectral local category} we describe the local category on the spectral side.
 \item In \S \ref{arcspaces} we discuss loop spaces and their singularities and describe the local category on the automorphic side (using infinite type sheaf theory as in Appendix~\ref{infinite type}).
 \item In \S \ref{Sarcspace} we study the concrete description of the category of constructible sheaves on $X_F/G_O$ in the ``placid'' case. 

 \item In  \S \ref{normalized-local}  we discuss the geometric analogue of ``unitary normalization'' of the $G$-action on $X$,
 which simply involves including appropriate Tate and cohomological shifts. 
 
 \item  \S \ref{Slocalconjecture} formulates the local conjecture and some of its consequences, and
\item  \S \ref{basic examples}  discusses some examples in which the conjecture is known,  including pointers to the recent literature on the subject.
 
     \end{itemize}
 
 
  


 

\begin{remark} 
On the side of $X$, it is interesting to relax the requirement that $X$ be smooth, and work within the broader class of affine spherical varieties. In this setting, calculations of ``IC functions'' in \cite{BFGM, BNS, SaWang}  suggest a generalization of the conjecture that follows, by dropping the coisotropic condition on $\check M$ on the spectral side. However, we do not know how to formulate the categorical conjecture at this point -- or whether singular spherical varieties are even the correct objects to consider. (In the singular toric case, for example, it seems that one could replace singular toric varieties by smooth toric stacks.) 
\end{remark}

 



 
 \subsection{The spectral local category}\label{spectral local category}
 In this section we highlight some features of the local category $\QCshear(\Mv/\Gv)$ on the spectral side. Recall (\S \ref{uld setup})
 that we are considering a smooth affine variety $\Mv$ equipped with a graded Hamiltonian $\Gv$-action, with $\GGm$-equivariant moment map $\mu:\Mv\to \fgxv$. We will default to using the \emph{neutral} grading on $\check{M}$ (see \S \ref{Sneutral}), and comment later (\S \ref{unnormalized local})  on the effect of changing the grading.   Correspondingly, as is appropriate for the neutral grading, the $\GGm$ action on $\check{G}$ itself is trivial. 
 
 We will make free use of the notions of shearing from \S \ref{shearingsec0};
 see in particular \S \ref{Mshear1}, which we briefly recall: The $\GGm$-graded ring
 $\cO_{\Mv}$ can be sheared to give $\cO_{\Mv}^{\shear}$, 
 a differential graded ring with zero differentials.
 When it is relevant (for example, in taking traces, cf. \S \ref{supersloppy}), we always consider
$\mathcal{O}_{\Mv}$ as a {\em super-} DGA whose $\Z/2$ grading is the reduction
of the integral $\Gm$ grading.
 With this convention, $\mathcal{O}_{\Mv}^{\shear}$ is commutative {\em as a super-DGA};
 it may not be 
 be commutative as a DGA if we naively ignored the super-structure.
 
The local spectral category $\QCshear(\Mv)$ can be described as the associated category of differential graded modules, which
  by the discussion and notations of \S \ref{shearingsec0}, 
  can also be described as the sheared category of modules for $\cO_{\Mv}$ itself.
 Again, there is a shearing functor $E \mapsto E^{\shear}$: a $\GGm$-graded complex $E$ of $\cO_{\Mv}$-modules
 gives a complex 
 $E^{\shear}$ of $\cO_{\Mv}^{\shear}$-modules, by shifting the
cohomological grading by the $\GGm$-grading; and the same is true adding $\check{G}$-equivariance everywhere. 
 
 \begin{remark} \label{Vxlocalconjecture}  
 Recall  (\S \ref{Slodowy}, \S \ref{NTmov}) that
  $\check{M}$ has the structure of vector bundle
  over $\check{G}/\check{G}_X$
  with fiber $V_X$, a certain graded $\check{G}_X$-representation
  that has been discussed in the cited sections.
  It follows that the local category may be described in terms of $(V_X, \check{G}_X)$ rather than $(\check{M}, \check{G})$, 
  \begin{equation} \label{Vxlc2}
\QCshear(\Mv/\Gv)\simeq \QCshear(\check{V}_X/\GvX). 
  \end{equation}
where the grading on $\check{V}_X$ has been defined e.g.\ at the start of \S \ref{NTmov}.
   \end{remark}

\subsubsection{Hecke action}
The equivariant moment map $\mu:\Mv/\Gv\to \fgxv/\Gv$ endows the category of equivariant sheaves on $\Mv$ with a tensor action of sheaves on the coadjoint representation. The $\GGm$-equivariance of the moment map allows us to shear this structure, so we find that $\QCshear(\Mv/\Gv)$ is a module category for $(\QCshear(\fgxv/\Gv),\otimes)$ -- i.e., for the spherical Hecke category as it appears on the spectral side in Theorem~\ref{Satake thm}.

\subsubsection{Affineness} \label{Spectralaffineness}
The affineness of $\Mv$ ensures that $\Mv/\Gv$ is affine over $\fgxv/\Gv$. It follows that $\QC(\Mv/\Gv)$ is identified with the category of modules for the algebra object $\mu_*\cO\in \QC(\fgxv/\Gv)$, and similarly for the sheared version: 
$$\QCshear(\Mv/\Gv)\simeq \mu_*\cO^{\shear}\module_{\QCshear(\fgxv/\Gv)}.$$
Another perspective on this is that $\QCshear(\Mv/\Gv)$ is generated by the structure sheaf as a Hecke-module category. 
More concretely, 
a representation $V$ of $\check{G}$ defines a $\check G \times \GGm$-equivariant
sheaf $\underline{V}$ on $\check M$, i.e., we tensor $V$ (with trivial $\GGm$-action)
with the structure sheaf of $\check M$. The affineness then guarantees that the resulting objects generate $\QCshear(\Mv/\Gv)$. Moreover the spaces of morphisms are explicit and readily computable:
\begin{eqnarray*}
\Hom(\underline{V},\underline{W})&\simeq&  
  \Hom^{\Gv}(\Hom(V,W),\cO_{\Mv}^\shear)\\
&\simeq& \Hom^{\GvX}(\Hom(V, W), \mathcal{O}_{\check{V}_X}^{\shear}),\end{eqnarray*}
cf. \eqref{Vxlc2}. 


\subsection{The automorphic local category}  \label{arcspaces}\label{automorphic local}

In this section we will assign to  a (untwisted) polarized hyperspherical variety $M=T^*X$, a category\index{$\mathcal{H}^X$} \index{$\mathcal{H}^X_G$}
$$  \mathcal{H}_G^X := \mbox{``$G_O$-equivariant sheaves on $X_F$''}$$
that we will call the ``$X$-Hecke'' or ``$X$-spherical'' category;
  sometimes we will write this simply as $\mathcal{H}^X$, although formally it depends both on $X$ and $G$
  as well as the specifics of the sheaf theory. 
  As usual it will have a small version $\mathcal{H}^X$ and a large version $\overline{\mathcal{H}^X}$.  
  This category will be equipped with a basic object and a Hecke action (\S \ref{Hecke action HGX}).
 \begin{quote}
   {\bf Caveat: some of the features of these sheaf categories, in particular safety/renormalization, are not adequately covered in the literature and should be taken as being provisional.}\footnote{At present, our
  reference for this material is the paper \cite{raskininfinite}. However, it is not yet published, and it  does not discuss either {\'e}tale/Betti contexts
   or safety and renormalization. We have formulated the Caveat simply to encourage further explication and study of the foundations of the theory.}
\end{quote}

 
The Caveat above is not ``serious,'' that is to say, we anticipate
that the relevant definitions and formalism can be filled in
with existing technology. 
However, it is adjacent to a ``serious'' issue: 
 we have given definitions that, in general, are, at least {\em a priori} completely impractical to compute with.
 The main issue is that $X_F$ is defined as a union of limits of schemes that are {\em singular}; 
 this problem arises in much work on arc spaces, when $X$ is singular, but it also appears for smooth $X$ when one considers strata in the loop space of $X$.  
 Although, as we will see below, there is a reasonable formal definition of the category of sheaves on $X_F$,
 this issue  prevents us from having a  concrete description of it, 
 as well as access to Verdier duality and the function-sheaf dictionary (see \S \ref{Sheafdesiderata} for some specific expectations which it would be good to prove).  
 We do not know how to resolve these issues in complete generality, 
 and regard this as a fundamental question for further study. 

However, there are two situations where many of these issues go away. Firstly, as described in the subsequent \S \ref{placid case},
$X_F$ is ``placid'' in many situations of interest, which permits
a much more explicit analysis of the sheaf categories. 
And, secondly, as we shall explain in the following section \S \ref{PlancherelCoulomb}, a substantial part of the
general conjecture (namely, everything related to the basic object) can always be reduced to a placid situation: arc spaces of smooth affine varieties.
 
 The contents of the current subsection are as follows:




\begin{itemize}
\item \S \ref{arc loop space} discusses arc and loop spaces and in particular illustrates
by example the singularities of $X_F$. 

\item \S \ref{XFsheaves}
 we outline the formal properties of categories of sheaves on loop spaces $X_F$ for $X$ an affine $G$-variety.
 These sheaf categories are defined
  formally, see Appendix~\ref{infinite type}.
  
  \item   \S \ref{XFGOsheaves}
describes the category of equivariant sheaves of interest, i.e., sheaves on $X_F/G_O$. 
  
  \item Definition \ref{basic object} and  \S \ref{Hecke action HGX} construct, respectively,  the basic object and the  Hecke action on sheaves on $X_F/G_O$. 
  
  These are  consequences of the general functoriality of sheaf categories on infinite type schemes and  
stacks~\cite{raskininfinite}, which we review in Appendix~\ref{infinite type}.
   \item  In \S \ref{subsec generalizations} we will briefly discuss the case of twisted polarizations and the unpolarized case. 
    

\end{itemize}
 







\subsubsection{Arc and loop spaces} \label{arc loop space} For the moment let $X$ be an arbitrary affine $G$-variety defined
over $\FF$, although our case of primary interest is when $X$ arises from polarizing a hyperspherical $G$-variety.

 The
 arc space
 $X_O$ is the scheme representing the functor that
 sends a test $\FF$-ring $R$ to $X(R[[t]])$,
 see \cite[2.2.1]{KapranovVasserot}. 
  This is represented as an inverse limit of the schemes
$$X_O = \varprojlim X_n,$$
where 
$X_n$ represents the functor $X(R[t]/t^n)$.
For $X$ affine, $X_O$ and the $X_n$ are all affine.
For $X$ smooth, $X_O$ is pro-smooth: the morphisms $X_{n+1} \rightarrow X_n$
are in fact vector bundles of dimension $(\dim X)$.


 
 
 The loop space $X_F$ is the ind-scheme representing the functor that sends a test $\FF$-ring $R$ to $X(R((t)))$, see \cite[\S 2.5]{KapranovVasserot}. 
    We can write it as a colimit of schemes $X^l$, $l\in \mathbb Z$, by fixing a $G$-equivariant embedding $X \hookrightarrow V$ into the space of a $G$-representation, 
  and taking $X^l$ to be the points of $X_F$ that lie inside $t^{-l} V[[z]]$
  (where we write $V[[z]]$ for the $R[[z]]$ points of $V$).
   
 
  Unfortunately the behavior of the $X^l$ is in general much less nice than
  $X_O$, even if $X$ is itself smooth. 
  In particular, the natural presentation of 
  $X^l$ as a projective limit is not placid:
  if we write  
 $$ X^l = \varprojlim X^l_n$$
 where $X^l_n$ is analogously defined
 i.e., as elements $t^{-l} v$
 where $v \in V[[z]]/t^{n+1} V[[z]]$
satisfies the equations defining $X^l$, rewritten in terms of $v$, modulo terms of order $n+1$. 
Typically,  $X^l$ are not smooth and the transition
 maps are not smooth, no matter how large $n$ is. 
 To illustrate both the complexity and interest of the situation we discuss a simple example. 
 
 \begin{example} \label{quadric}
Consider the case of $X$ a
 sphere inside a vector space $V$, i.e., the level set $Q=1$ of a quadratic form. 
 Taking a basis $e_0, \dots, e_n$
 we take $Q$ to be given by
 $Q(\sum x_i e_i) = x_0^2   +q(x_1, \dots, x_n)$, 
 for a nondegenerate quadratic form $q$ in $n$ variables. 
 Then $X^{-1}_n$ is identified
 with  the locus of $(v_0, \dots, v_n) \in V$ satisfying
\begin{equation} \label{Qprez} Q(v_0 + v_1 t + \dots v_n t^n) = t^2 + O(t^{n+1}).\end{equation}
 For $n=1$ we get simply pairs
 $(v_0, v_1)$ where $Q(v_0) =0 $ and $v_0 \perp v_1$,
 in particular, a smooth variety, 
  but the situation becomes more complicated at the next stage:
  The fiber of $X^{-1}_2 \rightarrow X^{-1}_1$ is $(\dim X)$-dimensional
over each $(v_0, v_1)$ with $v_0 \neq 0$. Over the fiber with $v_0 = 0$,
however, the map is not even surjective at the level of points:
its image is the locus $Q(v_1)=1$, and each fiber above this codimension 
$1$ set is now $(\dim X+1)$-dimensional.  
The same general pattern for transition maps holds at each higher stage
$X^{-1}_{n+1} \rightarrow X^{-1}_n$ -- they fail to be surjective, and
the fibre dimension jumps along the image. 
 
 
 Nonetheless, there are nice features to the situation.
 As proved in \cite{GK, DrFormalArc} 
 the singularities are ``locally finite dimensional''. 
For example, look at the singularity of $X^{-1}$
 at the constant arc $\gamma(t)=te_0$, 
which projects in \eqref{Qprez} to  $v_0=0, v_1 = \mbox{first coordinate vector}, v_2=v_3=\dots=0$. 
It can be checked that 
\begin{equation} \label{FNQ} \mbox{formal neighbourhood of $\gamma$ in $X^{-1}$ } \simeq \mathbb{A}^{\infty}
 \times \{q=0\},\end{equation}
 that is the local singularity structure is a quadric cone in one fewer dimension.
  \label{finitetypemodels}
  It is not a coincidence that this singularity is the
  same as the singularity of  the variety we get if we set $v_2=v_3=\dots= 0$, i.e., if
  we look just at  $\{v_0, v_1: Q(v_0 + v_1 t) = t^2\}$. This is a simple example
  of a global model (in this case, maps from $\mathbb{A}^1$ to $X$
  of degree $\leq 1$) modelling the singularities of a local situation (in this case,
  maps from the formal disc to $X$).
  It is possible that such techniques could provide concrete methods of accessing
  the sheaf theory on $X_F/G_O$ in the situations of interest to us.   
 \end{example}
 
 
 \subsubsection{Sheaves on $X_F$} \label{XFsheaves} 
As elsewhere in the paper, there are different choices for 
sheaf theory. Of relevance
for us in the current discussion are de Rham and {\'e}tale, although
in practice which one we choose makes very little difference in the local setting,
and for this reason we will not formally include superscripts ``dR, {\'e}t'' to 
indicate which one we are working with.\footnote{As mentioned in \S \ref{infinite type} the Betti sheaf theory presents challenges in infinite type, though in practice for stacks such as $X_F/G_O$ the Betti theory is expected to be well defined and produce the same categories as the de Rham theory.}
 
  As explained in  Appendix~\ref{infinite type},
working with either de Rham or {\'e}tale notions of sheaf theory\footnote{As explained in {\it loc. cit.}, to have small sheaf categories and ind-proper functoriality in the de Rham setting we have to restrict to a constructible setting, e.g., to ind-holonomic sheaves, though in our intended applications the discreteness of $G_O$-orbits discussed below makes the distinction between ind-holonomic and all $D$-modules disappear.},  we have -- by formally extending from the case of finite type schemes -- 
 \begin{itemize}
 \item Assignments  
 $$Z \leadsto \SHV(Z)=\SHV^!(Z), \SHV^!_s(Z), \Shv^!(Z)$$ for any scheme, stack or prestack of infinite type. Here we use $!$-sheaves by default and omit the $!$-notation when convenient. Recall that the categories of $*$-sheaves are canonically dual to those of $!$-sheaves whenever they are dualizable.  
\item  This is a contravariant functor under $!$-pullbacks, and covariant under ind-proper morphisms. We denote the pushforward functor as $f_*$ and note it is identified as a left adjoint of $f^!$. 
  

 \item  These functors satisfy base change, in the strong sense that they define a functor out of the correspondence category of prestacks (with one leg ind-proper).
 \item For schemes $X$ and affine groups $G$ the category is compactly generated by finite objects (i.e., equivariant constructible sheaves) $\SHV^!(Z)=\Ind(\Shv^!(Z))$
 where $Z=X/G$. 
\end{itemize}

In particular this formalism can be applied to $Z=X_O$ or $Z=X_F$.
The former setting of $Z=X_O$ is particularly nice.
Since $X$ is smooth, $X_O$ is pro-smooth, in particular {\em placid} (see Appendix \ref{appendix placid setting}); it follows that $!$- and $*$-sheaves on $X_O$ are identified, in such a way that the dualizing sheaf $\omega_{X_O}\in \SHV^!(X_O)$ is sent to the constant sheaf $\kk_{X_O}\in \SHV^*(X_O)$. 

\subsubsection{Sheaves on $X_F/G_O$} \label{XFGOsheaves} 
    
 The loop group ind-scheme $G_F$ acts on $X_F$. We will primarily be interested in the quotient $X_F/G_O$ by the arc-group, and specifically when $X$ is an affine spherical variety.  
  Let us first discuss what kind of object $X_F/G_O$ actually is.
  
 There are [at least] two distinct objects that deserve to go by the name $X_F/G_O$: the quotient {\em prestack} and the quotient {\em stack}. Recall that a prestack is merely a functor on derived commutative rings valued in simplicial sets (or synonymously, at the $\infty$-category level at which we work, topological spaces or higher groupoids). There is a natural notion of quotient prestack of a functor such as $X_F$ by a group functor such as $G_O$, which is described as 
 pointwise taking the simplicial set determined by the $G_O(R)$ action on $X_F(R)$.   

 
 
 
 On the other hand, we have the quotient {\em stack}, which is the (fppf) sheafification of this functor. Both objects are attached categories of $!$-sheaves by the general mechanism of right Kan extension. However it is reassuring to point out that categories of sheaves which satisfy descent for a given topology (say fppf) are not affected by replacing a prestack by its fppf sheafification. Thus in fact it follows from the results of~\cite{raskininfinite} - specifically the $h$-descent theorem for $!$-sheaves (~\cite[Proposition 3.8.1]{raskininfinite}) - that the two notions agree.
 
 From our point of view, the fundamental object of interest is the action itself and the resulting category of equivariant sheaves $\SHV(X_F)^{G_O}$ (as discussed in particular in~\cite[Section 3.9]{raskininfinite}). One can verify (extending~\cite[Proposition 3.9.2]{raskininfinite}) that this category agrees with that attached to the prestack or stack quotients $X_F/G_O$. Note that the morphism $X_F\to X_F/G_O$ is not itself finitely presented, but by factoring it as a quotient by a prounipotent group (for which equivariant $D$-modules form a full subcategory) and a reductive group (which is fppf) one can establish descent along this morphism directly.  
 
 In summary,
 sheaves on $X_F/G_O$ are understood to be ($!$-)sheaves on the quotient prestack $X_F/G_O$,
 and this agrees with all  other reasonable ways of defining the same concept:  
 $$ \overline{\mathcal{H}^X} = \SHV(X_F/G_O),
 \mathcal{H}^X =\Shv(X_F/G_O).$$
 
 As we discuss in Remark~\ref{! vs * conjecture}, we expect the theories of $*$- and $!$-sheaves on $X_F/G_O$ to be equivalent, and indeed such an equivalence is implied by Conjecture~\ref{local conjecture}. However we do not know how to see this directly.
 
 
 \begin{remark}
 Despite the fact that objects appearing seem (indeed, are) enormous, 
the problem of describing the entire category $\SHV(X_F/G_O)$ is actually rather concrete  and has very little of infinite nature in it. Namely, each of the countable strata of $X_F/G_O$ has the form $B \mathcal{G}$
 for a certain pro-group $\mathcal{G}_i$ which can be replaced (for the purpose of sheaf theory)
 with a finite dimensional reductive quotient $\overline{\mathcal{G}}_i$.  Thus
 the sheaf theory on each stratum is extremely simple; the only question
 is how these are to be glued. 
 \end{remark}
 
 \begin{remark}
   From the point of view of classical harmonic analysis, we might loosely think of
 $\Shv(X_F/G_O)$ as categorifying $G(\mathfrak o)$-invariant Schwartz functions,
 whereas $\SHV(X_F/G_O)$  categorifies distributions or generalized functions.
 See Example \ref{A1example1.5}. 
 \end{remark}

  A crucial feature of this setting is the {\em discreteness of $G_O$-orbits},   (see e.g.~\cite{GaitsgoryNadler}):   \begin{quote} \label{spherical is discrete} 
 {\em Discreteness of $G_O$-orbits:} For an affine {\em spherical} $G$-variety $X$, there are only countably many $G_O$-orbits on $X_F$. 
\end{quote}

  Thanks to this, we expect  all $D$-modules on $X_F/G_O$ to be ind-holonomic and all Betti sheaves to be ind-constructible, 
  and we expect   the de Rham and constructible sheaf theories to give equivalent categories (all three settings $\Shv, \SHV, \SHV_s$).
  Moreover, although we did not define Betti categories in 
 Appendix~\ref{infinite type}, it is reasonable to use the constructible categories
 here as the {\em definition} of the Betti category. 
Finally, we have access to the  full functoriality of constructible sheaves, which makes the situation considerably more tame than for example sheaf theory on $X_F$ itself.

 
  
 \subsubsection{Basic object and Hecke actions} \label{Hecke action HGX}
  We now describe some basic properties of the category $\mathcal{H}^X$,
  namely the basic object and the Hecke action. 
  
   \index{basic object}
 \begin{definition} \label{basic object}
 The {\em basic object} $\delta_X\in \Shv(X_F/G_O)$ is the pushforward to the loop space of the dualizing sheaf\footnote{
 Equivalently, with reference to the equivalence of $!$- and $*$-sheaves on the placid scheme $X_O$, the {\em constant} $*$-sheaf} on the arc space, i.e., for $i:X_O/G_O\hookrightarrow X_F/G_O$ we have $$\delta_X=i_*\underline{\omega_{X_O}}.$$  
 \end{definition}
  
  
Let us recall some general formalism about Hecke actions. 
The Hecke stack  $$Hecke:=BG_O \times_{BG_F} BG_O= G_O\backslash G_F/G_O$$ can be considered as an {\em ind-proper groupoid} over $BG_O$ (see~\cite[Sections II.2.5.1, III.3.6.3, V.3.4]{GR}).  Recall that a groupoid object over $S$ is a simplicial object $\cG_\bullet$ satisfying a Segal condition resulting in an identification of the simplices with iterated fiber products:
 \begin{equation*}
 \xymatrix{\cdots \ar[r]<1ex> \ar[r]<.5ex> \ar[r] \ar[r]<-.5ex> \ar[r]<-1ex> &
 \cG\times_S \cG\times_S \cG \ar[r]<.75ex> \ar[r]<.25ex> \ar[r]<-.25ex> \ar[r]<-.75ex> &
 \cG\times_S \cG \ar[r]<.5ex> \ar[r] \ar[r]<-.5ex> &
 \cG \ar[r]<.25ex> \ar[r]<-.25ex>&
 S}
 \end{equation*} 
 The Hecke groupoid is an ind-proper groupoid, meaning that all of the structure maps involved are ind-proper. For any prestack $Z$ with $G_F$-action, the quotient $Z/G_O\to BG_O$ carries a tautological action of the Hecke groupoid (the descent data describing $Z/G_O\to Z/G_F$). 
Our three flavors of sheaf theory ($\Shv,\SHV_s,$ and $\SHV$) evaluate on $Hecke$ to produce three flavors of Hecke categores. 
 
 The $G$-action on $X$ induces an action of the group ind-scheme $G_F$ on $X_F$, and thus the quotient stack $X_F/G_O\to BG_O$ carries an action of the Hecke groupoid. Again the functoriality of $\SHV$ automatically endows $\SHV(X_F/G_O)$ with the structure of $\overline{\Hecke_G}$-module category. 
  
  
\begin{remark} 
[Self-adjointness]
It is useful to note that the action of the Hecke category on any module category, in particular on $\SHV(X_F/G_O)$, is self-adjoint, in the sense of isomorphisms
 $$ \Hom(T_V \star \mathcal{F}, \mathcal{G}) \simeq \Hom(\mathcal{F}, T_{V*}\star \mathcal{G})$$
 for $V \in \Rep(G)$, this isomorphism being natural in $\mathcal{F}$ and $\mathcal{G}$. This is a formal consequence of the dualizability of the objects $T_V$ (with duals $T_{V*}$) and more generally is part of the powerful duality package available for modules over {\em rigid} tensor categories such as $\Hecke_G$ (see e.g.~\cite[Section 1.9]{GR}).
\end{remark}

\begin{remark}[Signs]
The Hecke action corresponds, under sheaf function correspondence
when applicable, to the action arising from the action of $G_{\mathfrak{f}}$
on functions on $X_{\mathfrak{f}}$ wherein $g \in G_{\mathfrak{f}}$
sends $f$ to the function $x \mapsto f(xg)$.
\end{remark} 
 
 
 
  
 \subsubsection{Generalizations} \label{subsec generalizations}
 
 It is our expectation that one can make  satisfactory definitions analogous to $\mathcal{H}^X$ in the twisted case 
 or in the unpolarized case using existing technology. We briefly discuss
 these in turn. 
 
 
 \begin{remark} \label{twisted case}
(The case of twisted polarizations $M=T^*(X, \Psi)$).  
In the case of the Whittaker model, Gaitsgory \cite[\S 2]{Gaitsgory-Whittaker} has defined a local derived category of Whittaker sheaves on the affine Grassmannian (and, more generally, at quotients of arbitrary level of the loop space of $G$). The same definitions make sense in the general case of Whittaker induction. Namely given a $\Ga$-bundle $\Psi \rightarrow X$
one begins by constructing the category $\SHV(\Psi_F/G_O)$ of equivariant sheaves on $\Psi$; and
then, following \cite{Gaitsgory-Whittaker}, takes ``twisted coinvariants'' for the $\Ga_F$-action on this category. \end{remark}



 

 


\begin{remark} \label{unpolarized local}
 The non-polarizable case: it is evidently important to  extend the construction $X\leadsto \SHV(X_F/G_O)$ to non-polarizable 
 anomaly-free hyperspherical varieties $M$. 
Note that it is our expectation that the {\em normalized}  Hecke action, 
a twisting of \S \ref{Hecke action HGX} to be described in  \S \ref{normalized-local}, 
will extend to this situation, rather than the action of \S \ref{Hecke action HGX} itself.

In the case when $M$ is a symplectic vector space,
this amounts to studying 
 ``the unramified part of the geometric Weil representation.'' The possibility of such a construction is well-known to experts, although we do not know of an entirely satisfactory reference for our purposes. We describe two relevant works:
 
 For $G=$ the dual pair $\Sp_{2n}\times \SO_{2n}$ (with $M=$ the tensor product of their standard representations), the category analogous to $\Shv(X_F/G_O)$ was constructed by Lafforgue and Lysenko  \cite{LafforgueLysenko} (with an emphasis on the perverse objects), by geometrizing the Schr{\"o}dinger model and the canonical intertwining operators. On the other hand, Raskin \cite[\S 10]{Raskin-homological} has developed a general framework for describing $G_F$-actions on categories as (geometric analogs of) Harish-Chandra modules; this was applied in \cite[\S 2.3, 4]{RaskinNisyros} to modules for the Weyl algebra $\mathcal W$ associated to the symplectic space $M_F$, in order to define an action of $\mathcal H_G$ on $\mathcal W\mbox{-mod}^{G_O}$; here, $G$ can be any subgroup of $\Sp(M)$.
 
 \end{remark}
 
 

 
\subsection{Sheaves on loop spaces: the placid case} \label{Sarcspace} \label{placid case}


\subsubsection{Setup} \label{placid loop setup}
In many cases,
the geometry of $X_F/G_O$ is particularly nice,
and it admits the following presentation, enabling   
 one to avoid the subtle issues of singularities discussed in \S \ref{arcspaces}. There is:
 \begin{itemize}
 \item  an exhaustion $X_F = \varinjlim X^l$ of the
ind-scheme $X$, and a $G_O$-stable presentation of each $X^l$ as $\varprojlim_{n} X^l_n$, where
\item the $X^l_n$ are of finite type, and the transition maps $X^l_{n+1} \rightarrow X^l_n$ are
torsors for a unipotent group scheme, and 
\item   the $G_O$-action on $X^l_n$ 
factors through an action of some quotient $G_{N}$ on each $X^l_n$. 
\end{itemize}

Let us collectively refer to these properties as {\em the placid case}, although {\em a priori} it is slightly stronger
than $X_F$ being placid in the sense of the Appendix. 


 For example, in the case of $X=$ a vector space, the $X^l_n$ were constructed in 
\S \ref{arc loop space}.\footnote{One should note that the situation
is quite rich even in the case when $X$ is a vector space,
because  
 $G_O$-orbit closures can be singular even though $X_F$ is very simple, cf. Example \ref{GJexample}. }When $X$ is a 
reductive group $H$ (and $G$ is a subgroup of $H \times H$ acting by left and right multiplication)
we can take the $X^l$ to come from strata of the affine Grassmannian,
and the $X^l_n$ to arise from the cover arising from the kernel of $G_O \rightarrow G_{n+1}$. 
Although these conditions are {\em a priori} quite restrictive,  a surprising number of  hyperspherical cases satisfy them:

 \begin{itemize}
  \item  The  Godement-Jacquet and Iwasawa--Tate periods, $X=M_n$ as a $G = \GL_n \times \GL_n$-space;
\item More generally, any vectorial case, e.g.\ the Hecke period $X=\mathbb{A}^2$ as a $G=\SL_2$-space; 
 \item  The group period, $X=H$ as an $H \times H$-space (possibly twisted by an automorphism in one factor).
 \item The Rankin--Selberg period, $X=\GL_n$ as a $\GL_n \times \GL_{n-1}$ space;
 \item the case of $X=\GL_n \times \mathbb{A}^n$ as a $\GL_n \times \GL_n$-space;
 \item the Gross--Prasad period, $X=\mathrm{SO}_n$ as a $\SO_n \times \SO_{n-1}$-space.
 \end{itemize}
 

Indeed, it seems possible that the placidity  of $X_F$ for all smooth $X$ can be proved by the techniques of  Drinfeld \cite{DrinfeldInfinite}, 
cf. \cite[\S 8.1]{ChenNadler}. The details of this have not appeared in print at the time of typing this sentence. 
 
 

 
 
 The restriction to this placid setting allows us to describe the entire sheaf theory just in terms of 
 the notion of  sheaves on Artin stacks.
 The discussion of this section can be carried out in any of our sheaf-theoretic contexts, though we will be primarily concerned with the {\'e}tale sheaf theory of
$X_F/G_O$, since this version can be readily compared with numerical
statements in the finite characteristic case. Accordingly, we restrict the discussion to that setting to simplify notations. Thus the notation $\Shv$ denotes, by default, ``{\'e}tale sheaves,''
with constructibility or boundedness conditions to be specified.    However, we will freely use at later
points that the same discussion transposes to the de Rham theory.


\begin{quote}
{\bf Caveat: We expect
the proofs of the statements that follow in this section -- i.e.
various properties of the sheaf theory developed in \S 
\ref{automorphic local}, but restricted to the placid case -- 
 to be straighforward. However, we don't state them as theorems,   because of 
the fact, already noted, that sheaf theory in these contexts
is not clearly documented, and we prefer
to leave the credit for such statements 
to a paper which also develops the relevant foundations in detail,
across the various types of sheaf theory that we would like to access.}
\end{quote}


 


\subsubsection{Duality and integration}\label{Sheafdesiderata} 

The following properties should be straightforward to establish 
in the placid case. In fact, we expect that they hold in the general context
of spherical varieties,  but we don't know how to   establishing them
because of the issues of singularities mentioned.


\begin{itemize}
 
\item (Duality): The sheaf theory on $X_F/G_O$ is equipped with a Verdier duality satisfying $D \delta_X =\delta_X$
that is moreover compatible with that on the spherical category, i.e.
$D(T \star \mathcal{F}) \simeq (DT) \star (D \mathcal{F})$
(where the duality on the affine Grassmannian is normalized to 
preserve the identity of convolution). 


\item (Integration): In the case where $\mathbb{F}$ is the algebraic closure of a finite field,
if $\mathcal{F}, D\mathcal{G}$ are Weil sheaves with trace functions $f,g: X_{\mathfrak{f}}/G_{\mathfrak{o}} \rightarrow \kk$ we have
\begin{equation} \label{int formula desid} [ \Hom(\mathcal{F}, \mathcal{G})^{\vee} ]= \int_{X_{\mathfrak{f}}/G_{\mathfrak{o}}} f(x) g(x) |\omega|,\end{equation} 
for motivation see Lemma \ref{Homlemma}; 
we follow the convention that  $\omega$ is a $G$-eigenmeasure (\S \ref{eigencharacter}), and normalized according to  
\begin{equation} \label{measXOGO}
\mu(X(\fo)/G(\fo)) = q^{-\dim(X)+\dim(G)} \frac{|X(\mathbb{F}_q)|}{|G(\mathbb{F}_q)|},
\end{equation} 
\end{itemize}


 We will sketch below an explicit model for objects in the sheaf category
 and explain, with reference to this explicit model, why duality and integration statements hold. 

 
  


 
 


 
  
 
\subsubsection{Explication of $\mathcal{H}^X_G$.}
In the placid case, 
both objects and morphisms 
of $\mathcal{H}^X_G$ can be described in terms of finite-dimensional computations,
as we now recall. 

 With notation as in \S \ref{placid loop setup}
 write  $\bar{X}^l_n$ for the Artin stack
$$\bar{X}^l_n = X^l_n /G_{N}$$
 where $N$ is chosen so large that the $G_O$-action
factors through it -- the constructions that follow
will formally speaking depend on this choice, but
will be independent of it up to equivalence. 
Write  $\Shv^l_n$ for the category of constructible $l$-adic sheaves on this Artin stack.
While the notion of sheaves on an Artin stack can be of course
derived from the general formalism described in the Appendix,
it is also accessible in more direct ways as sheaves for the lisse-{\'e}tale topology,
see \cite{LO}. 
  
 Placidity
 implies, as in Appendix \ref{appendix placid setting}, that
 the category $\Shv(X_F/G_O)$ constructed previously is equivalent
 to the corresponding category defined via $*$-pullbacks. 
 Therefore, in what follows, we will freely work with the $*$-version. 
 
 
  The formal construction of the category of $*$-sheaves $\Shv(X_F/G_O)$ implies the existence of functors
\begin{equation} \label{placidinclusion} \Shv^l_n \longrightarrow \Shv(X_F/G_O).\end{equation}
Explicitly, these functors are given by applying the functoriality of $*$-sheaves (these are dual to the already noted
functoriality for $!$-sheaves, namely, $*$-pullback over arbitrary morphisms and $!$-pushforward over ind-proper morphisms)
  to the diagram
$$\xymatrix{X^l_n/G_N & \ar[l] X^l_n/G_O & \ar[l] X^l/G_O \ar[r] & X_F/G_O}$$
 This permits us to think of objects of $\Shv^l_n$ as objects
 in $\Shv(X_F/G_O)$. 
  In fact,
 the morphisms can also be computed in $\Shv^l_n$, as we will explain.
 There are functors 
\begin{equation} \label{ShiftLN} \Shv^l_{n} \rightarrow  \Shv^l_{n+1}, \,\,\, 
 \Shv^l_n \hookrightarrow \Shv^{l+1}_n.\end{equation} 
 which arise from pullback, and from pushforward-pullback, along the
  diagrams of (space, group acting) 
$$ (X^l_{n+1},  G_{N'}) \rightarrow (X^{l}_n, G_{N}), (X^l_n, G_{N}) \leftarrow (X^{l}_n, G_{N''}) \to (X^{l+1}_n, G_{N''}),$$
where $N', N''$ are chosen so that the relevant $G_O$-action factors through these quotients.
Because the kernel of maps $G_{n+1} \rightarrow G_n$
are abelian unipotent group schemes,
the functors of \eqref{ShiftLN} are in fact {\em fully faithful},
so long as  $N, N', N''$ are chosen sufficiently large. 
The space of maps, computed in $\Shv(X_F/G_O)$,
between (the image of)
 a sheaf $\mathcal{F}$ on $\bar{X}^l_n$ and (the image of) a sheaf
 $\mathcal{G}$ on $\bar{X}^{l'}_{n'}$ is obtained 
 by pulling back both to some common $\bar{X}^K_N$ and then considering
 $$   \varinjlim_K \varinjlim_N \Hom_{\bar{X}^K_N}(\mathcal{F}, \mathcal{G}).$$
 Here ``$\varinjlim$''  refers strictly to the homotopy colimit of representing complexes;
 however in the inner limit all the maps are eventually quasi-isomorphisms
 and similarly for the outer colimit; therefore, this can be computed simply
 by a termwise direct limit of representing complexes. 
 
 
 In terms of this discussion, the
 desiderata above 
 correspond to the following constructions:
 
 \begin{itemize}
\item
The Verdier duality functor on $\mathcal{H}^X_G$
is compatible with the Verdier duality on each $\Shv^l_n$
(where $n$ is sufficiently large relative to $n$), up to shift. 
  The shifts
 are determined up to an overall dimension constant fixed by requiring $$ D \delta_X = \delta_X.$$

 


\item 
 Also the integration formula \eqref{int formula desid}
follows, when $\mathcal{F}, \mathcal{G}$ arise from $\Shv^l_n$,  by applying  Lemma \ref{Homlemma}
applied to suitable $\bar{X}^K_N$. 
\end{itemize}

 
 
    
 
 \subsubsection{Examples} 

  
 
 \begin{example} \label{A1example1}
  Take $X= \mathbb{A}^1$ and $G =\mathbb{G}_m$ (the ``Iwasawa--Tate case''). 
 For a test ring $R$, we have
 $X^l_n(R) = t^{-l} R[t]/t^{n}$
and the $G_O=R[[t]]^{\times}$-action on it factors through
 $(R[t]/t^{n+l})^{\times}$,
 with the transition maps in $n$ being the obvious projections.
 
  Lett $\delta_l$ denote the constant sheaf (with its trivial $G_O$-equivariant structure) on $X^l$, twisted by $\left<l\right>$, i.e., 
 \begin{equation} \label{deltadef} \delta_l = \underline{k}_{X^l}\left<l\right>,\end{equation}
 By this, we mean the $*$-sheaf arising from
 the constant sheaf on any one of the truncations $X^l_n$, by means of \eqref{placidinclusion}. 
  The twist by $\left< l\right>$ is, of course, the standard weight-zero perverse normalization of the sheaves, if we declare the zeroth stratum to have ``dimension $0$.''  
 
 
 We then compute:
\begin{equation} \label{Deltadeltahom} \Hom({\delta_{l_1}}, {\delta_{l_2}}) \simeq  H^*(B\mathbb{G}_m)  \langle - d \rangle,\end{equation}
   where $d:=|\ell_1-\ell_2|$ is the absolute value of the difference. 
   Indeed, without the normalizing twist by $\langle l \rangle$, the $\Hom$-space
   would be $H^*(B\mathbb{G}_m)$ for $\ell_1 > \ell_2$ and $H^*(B\mathbb{G}_m) \langle -2d \rangle$ otherwise. 
   

 \end{example}

 
 



 
 


 
 

 
  
\begin{example} \label{A1example1.5} ($ \overline{\mathcal{H}^X}$ as distributions). 



Continue with the notation of Example \ref{A1example1}. 
There are morphisms
 $$ \underline{k}_{X^l} \rightarrow \underline{k}_{X^{l-1}}, \,\, \underline k_{X_l} \rightarrow \underline k_{X^{l+1}}\langle 2 \rangle,$$
the second arising from the inclusion of dualizing sheaves, which are trivial here (up to shifts).
There are corresponding maps of $G_O$-equivariant sheaves.
Let $\delta_0$ be the object of $\overline{\mathcal{H}^X}$ corresponding to 
taking the colimit along the first system, and $\mu$ the object that corresponds to colimit along the second system. 
Then $\delta_0$ and $\mu$ (with their evident Frobenius structures) are analogues of the Dirac delta function at $0$, and the Lebesgue measure, respectively.  

 Indeed, for a sheaf $\mathcal{F}$ on $X^l/G_O$
 considered in $\overline{\mathcal{H}^X}$ by means of \eqref{placidinclusion}, with corresponding function $f$ on $X^l(\mathfrak o)$, we 
 get by an application of \eqref{int formula desid}
 $$[ \Hom(\mathcal{F}, \delta_0)^{\vee} ]= f(0) \mu(X(\fo)/G(\fo)) \mbox{ and } [ \Hom(\mathcal{F}, \mu)^{\vee} ] = \int_{X(\ff)/G(\fo)} f(x) dx,$$
 where the latter measure is normalized according to \eqref{measXOGO}. 
(Of course, the price of this enlargement is that the large category $\SHV$ also contains many other ``large'' objects
that are much less familiar from harmonic analysis.)
\end{example}
 
    
  \begin{example}\label{GJexample} 
   We consider the case of   
 $$X=M_n=\mbox{$n \times n$ matrices}, G= \GL_n \times \GL_n,$$
 with action map $x\cdot (g_1, g_2) = g_1^{-1} x g_2$.
  This is, in the theory of automorphic forms, the ``Godement--Jacquet'' period.
  
Fix $0 \leq j \leq n$ and let $\mathcal T_j$ be the Hecke sheaf for $\GL_n$ 
  that corresponds to the representation $\wedge^j \mathrm{std}^*$ on the dual group, i.e.
  it is the intersection complex of the stratum of the affine Grassmannian for $\GL_n$
  that indexes subspaces of $t^{-1} O^n/O^n$ of dimension $j$. Of course, ``intersection complex,'' here, just means the constant sheaf twisted by $\langle j (n-j) \rangle $. 
  
  We think of it as a sheaf on the second copy of $\GL_n$ in $G$.  Then we readily compute  \begin{equation} \label{Ij1}  \mathcal T_j \star \delta_X = \mathrm{I}_j   \langle j(n-j) \rangle\end{equation} 
where $\mathrm{I}_j$ is a $\GL_n \times \GL_n$-equivariant sheaf on $M_{n,F}$, supported on $M_{n,O}$ and pulled back from $M_{n,O}/t M_{n,O} = M_n$,  
whose fiber at a matrix $S \in M_n$ is given by the cohomology of
the space of $j$-dimensional subspaces $E \subset \kk^n$
such that $S|_E = \{0\}$. 
 
  \end{example}
  

 
  


 




 
  
   
    
 




 
 \subsection{Normalized action of $G_F$} \label{normalized-local} 
 
 In order that our main conjecture 
 match appropriately with the  \emph{neutral} grading on $\check{M}$ (see \S \ref{Sneutral}), we
 need to introduce a cohomological shift to the action of $G_F$ on $\Shv(X_F)$ which, at the level of functions, corresponds to a normalized, unitary action on $L^2$-spaces. We will introduce this normalized version first, before explaining how to ``twist away'' the normalization by modifying the $\GGm$-action.
 
 
 
 Recall from the structure theorem (in the notation of \S \ref{dp}) that $X$ is an equivariant vector bundle over a homogeneous space of the form $HU\backslash G$:
  $$X = S^+\times^{HU} G.$$
  We will assume, as in \S \ref{eigencharacter}, 
  that $X$ admits a nowhere vanishing eigen-volume form $\omega$ with eigencharacter $$\eta: G \to \Gm.$$
  When $G, X$ are defined over a finite field $\FF_q$, taking complex absolute values induces a positive eigenmeasure $|\omega|$ on the points of $X$ over the local field $\ff = \FF_q((t))$. This gives rise to a Hilbert space completion $L^2(X(\ff), |\omega|)$ of the Schwartz space $\mathcal S(X(\ff))$, which furnishes a unitary representation of $G(\ff)$ under the \emph{normalized} action 
\begin{equation}\label{action-G-unitary}
 g\cdot f(x) = \sqrt{|\eta(g)|} f(xg).
\end{equation}




    We lift this normalized action to the level of loop spaces, as follows: the character $\eta$ gives a ``degree'' or ``valuation'' map 
   \begin{equation} \label{deg definition} \deg=\deg_\eta: G_F \to \Gm_F \xrightarrow{\val} \mathbb Z\end{equation}
   To be clear here about the convention: $t\in \Gm_F$ has valuation $1$.
At a categorical level, the normalized action can be described as the automorphic shearing $\cC\mapsto \cC^{\deg \shear}$ of categorical $G_F$-representations $\cC$ defined from the homomorphism $\deg$ as in Example~\ref{shearing categorical reps}.


   
   More explicitly,  this normalized action of $G_F$ on $\Shv(X_F)$ is defined by twisting the translation action of  $g\in G_F$ by $\left<\deg(g)\right>$, i.e., 
 \begin{equation}\label{eq:normalized-local}
  g\cdot \mathcal F:= g^*\mathcal F \left< \deg(g)\right>,
 \end{equation}
where $g^*$ denotes pullback by the (right) translation action,
and $\langle \dots \rangle$ is as in our standing conventions (cf. e.g.\ \S \ref{Sqrtqsuper}). 
 This induces a similar twisted action of the Hecke category $\mathcal H_G$ on $\mathcal H^X_G$. \footnote{
 The twisting of Hecke actions can be directly  described as a shearing operation as in Example~\ref{shearing categorical reps} and Remark~\ref{Satake for cocharacters}:
 Namely $\deg$ defines a map $G_O\backslash G_F/G_O\to B\Z$, hence endows a central action $$(\Loc(B\Z),\otimes)\simeq (\QC(\Gm),\ast)\longrightarrow \cZ(\Hecke_G)$$ of $\Gm$ on $\Hecke_G$, for which the underlying monoidal functor $\QC(\G_m)\to \Hecke_G$ is trivial. It follows that we obtain a shearing operation on $\Hecke_G$-modules, which doesn't change the underlying category. Applying this operation to the $\Hecke_G$-category $\Hecke^X$ recovers the normalized action.  }
 
 
 
 This twisted action is compatible with the numerical version.  If
 we are working over $\mathbb{F}_q$, and $\mathcal{F}$ is a Weil sheaf on $X_F/G_O$
 with associated trace function $f$, then
 $$ \mbox{trace function for $\mathcal T_V \star \mathcal{F}$} = T_V f$$
 where $\mathcal{T}_V$ is as in \eqref{TVcaldef}, 
 $T_V$ is the corresponding Hecke operator obtained by sheaf-function correspondence; on the right
 $T_V f$ is obtained by integrating the \emph{unitary} action \eqref{action-G-unitary} of $G(\ff)$ on $\mathcal S(X(\ff))$. 
  
 \begin{example} \label{A1example2} 

 In the Iwasawa--Tate case,  let $V_n$ be the representation $z\mapsto z^n$ of $\check G$;
 then
 $$ \mathcal T_{V_n} \star \delta_X = \delta_n$$
the latter object being described in Example \ref{A1example1}. 
 
  The associated
  function (under sheaf-function correspondence) is
  $q^{-n/2} 1_{t^{-n} \mathfrak o}$; it has $L^2$ norm independent of $n$. 
  Note in order to have this be valid without a sign $(-1)^n$
  the parity shifts embedded in $\langle n \rangle$ are important: $\delta_n$
is a  super-sheaf in parity $(-1)^n$.
  
By contrast, under the unnormalized action we would find instead
 that $\mathcal T_{V_n} \star \delta_X$ is  the sheaf $\underline k_{t^{-n} O}$. 

 
\end{example}

\begin{example} \label{GJexample1.5}
In the Godement-Jacquet case of Example \ref{GJexample}
 the character $\eta$ is given by $\eta(g_1, g_2)= (\det g_1)^{-n} (\det g_2)^n$. 
Then we have
$\deg \mathcal{T}_j=- jn$ and
 for the normalized action
\begin{equation} \label{Inormdef} 
\mathcal T_j \star \delta_X=  I_j \langle  -j^2 \rangle
\end{equation}
compare with \eqref{Ij1}. 


\end{example} 
 


\begin{remark}\label{remark-choice-eta}
The foregoing definitions depend  on the choice of eigenmeasure $\omega$.
As discussed more generally in
\S \ref{ssseigencharinocuous}, the validity of the conjectures that we will formulate does not depend on this choice of extension. 
Indeed, any two eigenmeasures $\omega, \omega'$ will differ by $\nu: X \to \Gm$,
and this defines an equivalence of categories between sheaves on $X_F$ with the $\eta$-normalized $G_F$-action and sheaves on $X_F$ with the $\eta'$-normalized $G_F$-action, given by applying a  twist by $\left< \val\, \nu \right>$. 
\end{remark}
 
 
 
  
 \subsection{The local unramified conjecture} \label{Msheaves}
 \label{Slocalconjecture}

In this section we introduce the local conjecture. We are in the setting of \S \ref{uld setup}, with $M=T^*X$ polarized and the dual $\Mv$ is endowed with the neutral $\GGm$-action. 
 
       \begin{conjecture} \label{local conjecture}
There is an equivalence of categories\footnote{As per our general conventions, ``small categories'' are small $\kk$-linear idempotent complete stable categories with exact functors, and ``large categories'' are $\kk$-linear presentable stable categories with colimit preserving functors.}:
\begin{itemize}
\item (small version):
$$\LL_X: \Shv(X_F/G_O)\longrightarrow  \mbox{perfect $\Gv$-equivariant modules for $\mathcal{O}_{\Mv}^{\shear}$}$$
\item (large version):
$$\LL_X: \SHV(X_F/G_O) \longrightarrow\QCshear(\Mv/\Gv).$$
\end{itemize}
The equivalence is required to be compatible with {\em pointings} (\S\ref{pointings}), {\em Hecke actions} (\S\ref{Hecke local conj}), {\em Galois actions} (\S \ref{Galois local conj}) and {\em Poisson structures} (\S\ref{Poisson local conj},  \S \ref{Poisson from loop}). 
\end{conjecture}


  

We now enumerate and briefly discuss a sequence of structures we require to match on the two sides and some of the immediate consequences.
Note that the left hand side of the conjecture depends on a choice of de Rham or {\'e}tale sheaf theory, but
the conjecture  says that this depends on that choice only through the coefficient field $\kk$. 

\subsubsection{Pointings.}\label{pointings}

The first requirement we make of the conjecture is a matching of basic objects on both sides, i.e., a ``pointing'' of the equivalence:

\begin{itemize}
\item[$\bullet$][Pointing.] There is an identification $\LL_X(\delta_X)\simeq \cO_{\Mv/\Gv}^\shear$ between the image of the basic object and the sheared structure sheaf of $\Mv/\Gv$. 
\end{itemize}

 For instance if we compute $\Hom(\delta_X, \delta_X)$ inside the category of sheaves on $X_O/G_O$, we should have
\begin{equation} \label{invquot}  
\mbox{sheared algebra of functions on $\Mv\sslash \Gv$} \stackrel{?}{=}  \End(\delta_X)   = H^*_{G}(X),
\end{equation}
 the $G$-equivariant cohomology of $X$; the grading on the left hand side is by the $\GGm$-action on $\Mv$.
This can be readily verified by hand in many examples. \footnote{
 Note that this includes a claim on the \emph{formality} of the endomorphism dg-algebra, i.e., the fact that it is quasi-isomorphic to its cohomology. In the homogeneous case, $X=H\backslash G$, this is the same as the cochain complex of $BH$, which is well-known to be formal, and canonically isomorphic to the ring of $\check H$-invariant polynomial functions on $\check{\mathfrak h}^*$, the dual Lie algebra of the dual group. The general case reduces to the homogeneous case, using the structure of a vector bundle $X\to H\backslash G$, i.e., $\End_{\text{Shv}(X/G)} \underline{k}_X = \End_{\text{Shv}(BH)} \underline{k}_{BH} = H^*(BH) = H^*_G(X)$.}
See also Example~\ref{multiplicity-freeness} where an elaboration of this calculation, combined with the compatibility of the local conjecture with Poisson structure, forces the multiplicity-freeness of the Hamiltonian space $\Mv$.  
 
 
 
\subsubsection{Hecke actions}\label{Hecke local conj}

Perhaps the most important requirement of the local conjecture is that it matches actions of the spherical Hecke category on both sides.
We first state a ``normalized'' form:
          
\begin{itemize}
\item[$\bullet$][Hecke actions]          
$\LL_X$ has the structure of equivalence of module categories for the spherical Hecke category $\Hecke_G$, where $\Hecke_G$ acts on the automorphic side by the normalized action as in \S \ref{normalized-local}\footnote{In particular, we are assuming a choice of square root of $q$ in $k$, whenever half-Tate twists appear. We will later present an unnormalized variant of our conjecture.} and on the spectral side via the
derived Satake isomorphism $\LL_G$, and the moment map
 $$ \check{M}/\check{G} \longrightarrow \fgv/\check{G}. $$
 \end{itemize}
 
 The Hecke-equivariance implies a very explicit knowledge of the automorphic category. Given a representation
$V$ of $\check{G}$ we have an equivariant vector bundle $\underline{V}\in \QCshear(\Mv/\Gv)$, and as noted in \S \ref{Spectralaffineness}, these objects generate and have explicitly computable Hom spaces. The matching objects on the automorphic sides are the 
sheaves $\mathcal T_V\star \delta_X$ 
on $X_F/G_O$ obtained by applying the corresponding Hecke operator to $\delta_X$ (under the unitarily normalized action). 
Under the sheaf-function correspondence, $\mathcal T_V \star \delta_X$
matches with the function $f_V$ obtained by applying the corresponding Hecke operator $T_{V}$
to $1_{X(\mathfrak o)}$. Thus the conjecture implies isomorphisms of complexes 
\begin{equation} \label{basic} \mathrm{Hom}(\mathcal T_V \star \delta_X, \mathcal T_W \star \delta_X) \simeq  \Hom^{\check G}(V, W \otimes \cO_{\Mv}^\shear),\end{equation} where the degree grading on the right hand side corresponds to the weight or cohomological grading on the left. 
Moreover these explicit Hom spaces (and their compositions) capture the entire automorphic category. In particular {\em all} sheaves on $X_F/G_O$ can be generated from the basic object through the action of Hecke functors. 

Note that the arc space $X_O$ is placid, and hence sheaf theory there is well behaved (for example satisfies Verdier duality). Thus the local conjecture guarantees that all sheaf theory on $X_F/G_O$ can be reduced using the Hecke action to inherently finite-dimensional calculations on $X_O$, and the potential subtleties of sheaf theory in the non-placid setting disappear.
 This is most succinctly expressed using the inner endomorphisms of the basic object -- {\em Plancherel algebra}, see \S\ref{PlancherelCoulomb}.
 
 \begin{remark}[$!$- vs $*$-sheaves]\label{! vs * conjecture} 
  Conjecture~\ref{local conjecture} provides an equivalence between the categories $\SHV^*(X_F/G_O)$ and $\SHV^!(X_F/G_O)$ of $*$- and $!$-sheaves on $X_F/G_O$, since the two sheaf theories are canonically dual and the category $\QCshear(\Mv/\Gv)$ is canonically self-dual. In fact this equivalence is naturally Hecke-equivariant, since the self-duality of $\QCshear(\Mv/\Gv)$ is linear over $\fgxv/\Gv$. It would be very interesting to have a direct proof of this equivalence, i.e., a construction of a $G_O$-equivariant renormalized dualizing sheaf on the (potentially) non-placid ind-scheme $X_F$. As we will discuss in \S \ref{automorphic-factorization} the $*$-sheaf theory is much more natural for the construction of the geometric form of $\Theta$-series and local-global compatibility for the ($!$-)period sheaf.   \end{remark}

\subsubsection{Changing $\GGm$-actions and the unnormalized conjecture.}\label{unnormalized local}
The local conjecture posits that the local automorphic category with the normalized Hecke action $\SHV(X_F/G_O)^{\deg \shear}$ --- sheared by the degree character of $G_F$ as in~\ref{shearing categorical reps} --- matches the local spectral category $\QC(\Mv/\Gv)^{\shear}$  where we shear using the {\em neutral} $\GGm$-action on $\Mv$. 


This conjecture is ``analytic'' or ``normalized'' in the parlance of \S \ref{analyticarithmetic}. 
We can pass to the ``arithmetic'' or ``unnormalized'' version using the compatibility under geometric Satake between characters of $G$ and central cocharacters of $\Gv$ (see Remark~\ref{Satake for cocharacters}). 
In particular, in this way,  we deduce forms of the conjecture where the action of $G_F$  on $\Shv(X_F)$ is given by usual translations (i.e., the unnormalized case).

For explicitness in what follows, let us write the neutral action explicitly as $\textrm{neut}$, so that the neutral shear
will be denoted $\QC(\Mv/\Gv)^{\textrm{neut}\shear}$.  
Shearing by $\eta$ to undo the degree shift
in the conjecture, we find an identification of
 $ \SHV(X_F/G_O)$
 with $\QC(\Mv/\Gv)^{(\textrm{neut}+\check\eta)\shear}$,
 where on the right
 where we have modified the $\GGm$-action by the central cocharacter $\check \eta$, i.e., we define a non-neutral action by letting $z\in \GGm$ act instead by the neutral action of $(\check \eta(z), z)\in \check G\times \GGm$.
\footnote{Here is a sign check. In the Iwasawa--Tate example of Example \ref{A1example1},  let $V$ be the standard representation, 
then $T_V$ is the Hecke operator corresponding to a uniformizer, and the unnormalized
$T_V \star \delta_0 =\delta_1 \langle -1 \rangle$ with our previous notation;
thus $\Hom(T_V \star \delta_X, \delta_X) =  \Hom(\delta_1 \langle -1 \rangle, \delta_0)
\simeq H^*(B\Gm)$. On the other hand, we can compute
$\Hom(V, \mathcal{O}(\Mv)^{\shear})$ with the arithmetic shearing as in Example
\ref{A1dualarithmeticshear}: it is again in $\GGm$ degrees $0,2,\dots$.}
 
 
 
 Now, on the right hand side, we can further shear by the action of $2\rho$ on {\em both $\Mv$ and $\Gv$}
 by \eqref{eqqq2} to get
$$ \SHV(X_F/G_O)  \simeq \QC(\Mv/\Gv)^{(\textrm{neut}+\check\eta)+2\rho \shear}.$$
 Note that, above, the $\GGm$ action on $\Mv$ is through $\textrm{neut}+\check{\eta}+2\rho$ --
 that is to say, the arithmetic shear described in \S \ref{Marithshear} -- 
and the $\GGm$ action on $\Gv$ is through $2\rho$. So we can abridge the above statement to:
 $$ \SHV(X_F/G_O) \simeq \QC(\Mv/\Gv)^{\textrm{arith.}  \shear},$$
which  is the unnormalized form of the local conjecture, written in a form to be compatible with the arithmetic
form of geometric Satake.
Again, we emphasize that on the right $\GGm$ is acting on {\em both} $\Mv$ and $\Gv$. 
We remark that the shearing operations above do not change the underlying categories -- just the Hecke actions on them.
 




 
  
  
  \subsubsection{Galois-linearity}\label{Galois local conj}
   If $\FF$ is the algebraic closure of a finite field
of size $q$, then we require that $\LL_X$ is Galois-linear: 



\begin{itemize}
\item[$\bullet$][Galois linearity]          
$\LL_X$ has the structure of Frobenius-equivariance, i.e., it intertwines the autoequivalence of $\mathcal H^X$ induced by Frobenius with  the ``analytic'' action of Frobenius (\S \ref{analytic-M}) on the spectral side.
 \end{itemize}


Note that, since we are supposing that $(G, M)$ is the ``distinguished split form'' hypothesized in \S \ref{goodhypersphericalpairs}, 
the expectation is that this analytic action on $\mathcal{O}_{\Mv}^{\shear}$ is simply the action which scales by $q^{i/2}$
in cohomological degree $i$. In the general case -- that is to say,
even if $(G, M)$ is not the distinguished split form -- this analytic action
 is a a finite order twist of this action, 
as constructed in \S \ref{CheckMRat}. 
We proceed with our discussion in the split case, leaving the modifications to the reader.


 


  The Galois-linearity  
  implies that $\LL_X$ takes Weil sheaves to $q^{1/2} \in \GGm$-equivariant sheaves, and for Weil sheaves $\cF,\cF'$ the Frobenius action
on the left hand side of
$$ \Hom(\mathcal{F},\mathcal{F}') \simeq \Hom(\LL_X(\cF), \LL_X(\cF'))$$
corresponds to the action of $q^{-1/2} \in \GGm$ on the right hand side.   
\footnote{
As a sign check consider the situation of \S \ref{pointings} when $\cF=\cF'=\delta_X$, 
  the basic
object with its trivial Frobenius-equivariant structure; the 
assertion is then that
the (geometric) Frobenius action on $H^*_G(X)$
coincides with the action of $1/\sqrt{q}$ on $\Gv$-invariant functions on $\Mv$.
The inverse seems strange but is in line with our conventions on shearing:
degree $k$ functions on $\Mv$ are sheared via a cohomological shift $[k]$
and a Tate twist of $(k/2)$. }
 
 
In fact,
the spectral side of the conjecture admits a natural graded lift $\QC(\Mv/\Gv\times \GGm)$, in which we impose in addition equivariance for $\GGm$. On the automorphic side, it is natural to expect this to match the category of constructible graded sheaves on $X_F/G_O$, as has been defined in the finite-dimensional setting in ~\cite{HoLiMixed}. The latter is roughly speaking obtained from the category of Weil sheaves by formally imposing that Frobenius acts by powers of $q$. This enhanced version of the Galois-linearity of the conjecture would generalize the ``Tate'' form of geometric Satake (as in~\cite{xinwenSatake}), and imply that the geometry of spherical varieties enjoys some of the very special mixed geometry (or ``Tate-ness'') of flag varieties. 


\subsubsection{Parity and spin structures.}
Following the general discussion of \S \ref{supersloppy}
the conjecture has a version where, on both sides, 
  we take sheaves of super-vector spaces.  The parity constraint, where
we use the parity element $z_X$ from \eqref{zXdef}, should be the following:

\begin{itemize}
\item[$\bullet$][Parity]: 
  even sheaves on the left side are carried to sheaves of parity   $z_X$ (i.e.,
super-sheaves whose parity coincides with the action of $z_X$). 
\end{itemize}

That is to say: we consider  $\check{G}$-equivariant sheaf on $\check{M}$
whose super-grading coincides with the grading defined by the central involution $z_X \in \check{G}$. 
 

Here are some examples:

\begin{itemize}
 \item The basic sheaf $\delta_X$. It is itself even,
 and it is sent to $\mathcal{O}_{\Mv}$; the parity 
 condition of \S \ref{parity} implies that $(z_X, -1)$ acts trivially on it;
 that says precisely that it has parity coinciding with the action of $z_X$.
 
 
 \item  The parity of $T_V \star \delta_X$
 is determined by the action of $z_X$ on $V$, e.g.
 if $z_X$ acts as $1$ on $V$ then $T_V \star \delta_X$
 is even. 
 
  To see this, recall that
 the parity of $T_V$ itself is, by our conventions, described
 by the action of $(-1)^{2 \rho}$ on $V$, and the convolution
 introduces a twist $\langle \deg T_V \rangle$ which alters the parity
 through the action of $(-1)^{\eta}$ on $V$. 
 
 
 On the spectral side, the action of $z_X$
  on $V \otimes \mathcal{O}_{\Mv}^{\shear}$ 
  is the diagonal action. If $z_X$ acts by $1$ on $V$,
  its diagonal action here then coincides with the action of $-1 \in \GGm$, as desired. 
  
 
  \end{itemize}
  
  
  

\begin{remark}[Dependence on spin structures.]\label{local conjecture depends on spin}
We have formulated the local conjecture in the presence of a local coordinate, i.e., an identification $O=\FF[[t]]$. It is natural to ask for a version that is independent of the choice of coordinate, i.e., equivariant for actions of the group of automorphisms of the disc $D=Spec(O)$. Perhaps surprisingly, we do {\em not} expect the most straightforward coordinate-independent formulation of the local conjecture to hold in general. This is due to a need to twist by spin structures on the curve which we will encounter globally in the definitions of both period- (\S \ref{bunX} and \ref{spindep}) and L-sheaves (\S \ref{LsheafXnormalized} and \ref{Lspinindep}). We defer to \S \ref{local-global} for a precise formulation of this spin-twisted and coordinate-independent local conjecture.  
\end{remark}





\subsubsection{Arthur Parameters.} \label{spectral local Arthur}\
 A striking feature of the $L^2$ theory of
spherical varieties is that they are expected (see \cite{SV} and also \cite{ClozelBurger})
 to contain
only unitary representations of a {\em single} Arthur type,  that is,
they are all associated to a single conjugacy class of maps $\SL_2 \rightarrow \check{G}$. 
This $\SL_2$ is the one from which the dual $\check{M}$ is Whittaker-induced, 
see \eqref{ArthurSL2}. 

Let us examine some related phenomena
im the local conjecture. 
Denote by $(\varpi,f)$ the corresponding $\mathfrak  sl_2$-pair (\S \ref{sl2pair}).  
\begin{itemize}
\item[(a)]
The  moment map for $\Mv$ misses $\cNN_{<f}$, the union of nilpotent orbits smaller than $f$. 
Therefore, 
the local conjecture
implies that 
\begin{quote} $\SHV(X_F/G_O)$ is {\em $f$-antitempered as a $\Hecke_G$-module category},
\end{quote} 
by which we mean that 
 it is annihilated by the sheared structure sheaf $\cO^\shear_{\cNN_{<f}}\in \QCshear(\fgxv/\Gv)$.
  
\item[(b)] The second  point is a more direct parallel to the fact, in the classical setting,
that the archimedean size of Hecke eigenvalues is essentially controlled by $\varpi$.   The $\Rep(\Gv)$-action on $\SHV(X_F/G_O)$, by means of the Hecke action,
 factors through the  sheared forgetful functor $(-)^{\varpi\shear}: \Rep(\Gv)\to \Rep(Z_\Gv(\varpi))$,
 obtained by restricting along the inclusion $Z_{\Gv}(\varphi) \hookrightarrow \Gv$
 and then shearing by $\varpi$. 
\end{itemize}

Point (b) comes  from the construction of the $\GGm$-action on the Whittaker induction.   It is for example
familiar from the usual Satake isomorphism when $X$ is a point. In that case, the assertion amounts to the fact
that the cohomology functor on $\mathrm{Gr}_G$ corresponds 
to the forgetful functor, taking a representation of $\Gv$ to its underlying vector space,
but sheared through the action of $2 \rho$. 

 
 

 

\subsubsection{Singular support} 

We can also formulate a ``safe'' or ``nilpotent singular support'' version of the local conjecture. This version predicts an equivalence of categories
$$\SHV_s(X_F/G_O) \longrightarrow\QCshear_\cNN(\Mv/\Gv)$$ where we consider ind-safe sheaves on the automorphic side and sheaves supported over the nilpotent cone in $\fgxv/\Gv$ on the spectral side. This equivalence is required to be linear for the ``safe / nilpotent singular support'' form of the derived geometric Satake correspondence described in~\cite{ArinkinGaitsgory}.
 Indeed this version follows from the Hecke compatibility of the local conjecture as in Appendix \S \ref{safe Langlands}. Namely, we restrict both sides of the conjecture to the full subcategories which are torsion with respect to the action of the algebra $Z$ of endomorphisms of the unit in the Hecke category. 

  



\subsubsection{Poisson structure.}\label{Poisson local conj}
We will describe two closely related structures on the automorphic side which are expected to reflect the induced Poisson bracket on functions on $\Mv$: loop rotation and factorization. We formulate the simpler statement about loop rotation here (namely that the deformation given by loop-rotation equivariance recovers the Poisson structure on $\Mv$), spell it out more concretely in \S \ref{Poisson from loop}, 
and defer to \S \ref{automorphic-factorization} and \S \ref{spectral-factorization} for a discussion of factorization.

\begin{remark}  
The local conjecture implies that the  the entire automorphic category $\SHV(X_F/G_O)$ carries a variant of a braided tensor structure:
  the category generated by the basic object carries a {\em locally constant} factorization structure, which in the Betti setting is equivalent to a braided monoidal ($E_2$) structure, or {\em balanced} braided structure ({\em framed} $E_2$-algebra) when combined with loop rotation. 
\end{remark}

The loop spaces $X_F$ and $G_F$ carry compatible actions of $\Gm$, 
 which arise from the action of $\mathbb{G}_m$ on $\FF((t))$ via rescaling of the parameter $t$. These actions
 fix the arc spaces $X_O$ and $G_O$, and induce compatible actions of $\Gm$ on the monoidal category $\Hecke_G$ and its module category $\SHV(X_F/G_O)$.
 
 Thus we may consider the $\Gm$-equivariant category $$\SHV_u(X_F/G_O):=\SHV(X_F/G_O\rtimes \Gm)=\SHV(X_F/G_O)^{\Gm},$$ i.e., the strongly $\Gm$-equivariant objects in the $X$-spherical category. This is a $H^*_{\Gm}(\mbox{pt}, k) \simeq \kk[u]$-linear category, where $u$ has cohomological degree two, which specializes at $u=0$ to a full subcategory (the {\em equivariantizable objects}) of the original category,
 $$\SHV_u(X_F/G_O)\otimes_{\kk[u]}k\hookrightarrow \SHV(X_F/G_O).$$ (The fullness is a consequence of the Koszul duality of~\cite{GKM}, see e.g.~\cite[Proposition A.6]{BZCHN2}.) In other words, we have a canonical deformation of a full subcategory of the $X$-spherical category. 
 
 \begin{lemma} Conjecture~\ref{local conjecture} implies that all of $\SHV(X_F/G_O)$ is equivariantizable, $$\SHV_u(X_F/G_O)\otimes_{\kk[u]}k\simeq \SHV(X_F/G_O).$$ 
 \end{lemma}
 
 \begin{proof} For the spherical Hecke category $\Hecke_G$ itself the full subcategory of equivariantizable objects is the entire category. Since the basic object is naturally $\Gm$-equivariant, it follows that the full subcategory it generates under the Hecke action is equivariantizable as well.  
 The Lemma follows from the observation (\S \ref{Hecke local conj}) that in the presence of the local conjecture, the entire automorphic category is generated in this way.
\end{proof} 
 
We now require that under the local conjecture this $u$-deformation defines a deformation quantization of $\Mv/\Gv$ with its (sheared) Poisson bracket. We formulate here a very weak form of this requirement:


\begin{itemize}
\item[$\bullet$][Poisson structure]          
The Hochschild cohomology class of $\SHV(X_F/G_O)$ defined by the first-order data of the $u$-deformation $\SHV_u(X_F/G_O)$ is matched with the Hochschild cohomology class of $\QCshear(\Mv/\Gv)$ defined by the (sheared, 2-shifted) symplectic form.
 \end{itemize}

Note that the Hochschild classes in question are in fact in degree 0. Automorphically, the $u$-deformation is a deformation over $k[u]$ where $u$ has cohomological degree 2. Spectrally, since the symplectic form on $\Mv$ has $\GGm$-weight 2, the sheared bracket on $\cO^{\shear}(\Mv)$ has degree $-2$ (i.e., defines a $P_3$-structure) whence again a degree 0 Hochschild class.

The structure theory of hyperspherical varieties can be used to prescribe a canonical global $k[u]$-deformation quantization of $\Mv/\Gv$.
A stronger form of this compatibility requires this entire deformation to match the $u$-deformation of the automorphic category. This is formulated (using the language of Plancherel algebras) as Conjecture~\ref{noncommutative poisson conjecture} in the next section.





 
  
 \subsection{Examples} \label{basic examples}
Let us discuss several examples where at least some parts of  Conjecture~\ref{local conjecture} are known. 

 
\begin{example} \label{A1example3}
 We return to our  ``easy'' running example of $X=\mathbb{A}^1$ (see Example \ref{A1example1}, \ref{A1example1.5}, \ref{A1example2}). 
In this case one can verify the equivalence ``by hand,''
as we will essentially do below; we will also see what happens to the ``Dirac delta'' and ``Lebesgue'' sheafs 
from Example \ref{A1example2}. 

Here $\check{M}=T^* \mathbb{A}^1$.  
 In the normalized action, the $G^{\vee}=\Gm$ action
 on $\check{M}$ scales the $\mathbb{A}^1$-direction and antiscales the
 dual $T^* \mathbb{A}^1$-direction.
 Let $x$ be a coordinate on $\mathbb{A}^1$ and $\xi$ a dual coordinate on $T^* \mathbb{A}^1$, so that
 the $G^{\vee}$ action is given by $\lambda \cdot x=  \lambda^{-1} x, \lambda \cdot \xi = \lambda \xi$
 and the $\GGm$ action antiscales both; both $x,\xi$ are in cohomological degree $1$.
 
 We will write
 $[n]$ for the representation $z \mapsto z^n$ of $\check{G}$; the sheaf   $\delta_n$ introduced  in Exanple \ref{A1example1}
 corresponds to $[n] \otimes \mathcal{O}_{\check{M}}^{\shear}$.
 We have computed $\Hom(\delta_n, \delta_m)$ in \eqref{Deltadeltahom};
on the spectral side the same computation yields
 $$ \Hom([n] \otimes \mathcal{O}, [m] \otimes \mathcal{O}) = \Hom_{G^{\vee}}( [n-m] , \mathcal{O}).$$  
 The invariants in question are spanned by monomials $x^a \xi^b$ where $a,b \geq 0$ and $b-a = n-m$.
This lies in cohomological degree $a+b$.  That is to say, the $\Hom$-space
 is one-dimensional  in degrees $|n-m|, |n-m|+2, \dots$,  which matches with \eqref{Deltadeltahom}.
 
Let us also discuss what happens in the limit, to see where
the objects $\delta_0, \mu$ of Example \ref{A1example1.5} go. 
The {\em unnormalized} sheaf $k_{X^l}$ corresponds, on the spectral side, 
to $[l] \otimes \mathcal{O} \langle - l \rangle$,
which we can formally think of as $x^{-l} \mathcal{O}$. 
    The skyscraper at $0$ corresponds 
to taking a limit as $l \rightarrow -\infty$, which gives 
a $\mathcal{O}$-module which can be identified
with $\kk[x, x^{-1},\xi]$.  We can also take the limit of sheaves $k_{X^l}\langle 2l \rangle$
as $l \rightarrow \infty$, corresponding to $[l] \otimes \mathcal{O} \langle l \rangle$
or $\xi^{l} \mathcal{O}$, and get the object $\kk[x, \xi, \xi^{-1}]$.  It might be quite interesting
to study the images of other natural distributions on $X$, under the local conjecture,
in more general instances. 
 \end{example}

 

 
 
 
 
 
 









 


 
\subsubsection{The group case} \label{basic example: group}
 
 Here the space $X$ is a reductive group $H$ with a left and right action of $G=H \times H$; 
and the dual symplectic variety is  now $\Mv=T^\ast \Hv$ as a Hamiltonian $\Hv\times \Hv$-space
where the action of one factor is twisted by the duality involution. In particular, 
we have $\check{G}_X = \Hv$ and the space $V_X$ is 
the dual Lie algebra $(\mathfrak{h}^{\vee})^*$, placed in $\Gm$ weight $2$; 
thus, the conjecture 
 is precisely the derived Satake theorem of \cite{BezFink},
in the case of $\FF=\C$, 
which was recalled as Theorem \ref{Satake thm}.

Let us talk through the various desiderata: 
the requirement on pointings (\S\ref{pointings}) follows from the construction.
The statement about the equivalence
and Hecke actions (\S\ref{Hecke local conj})
{\em almost} follows from the monoidal nature of derived Satake,
but there is a subtlety:
one needs to know that the action of the
inversion map $H \to H$  is induced on the spectral side of $\LL_H$  by the {\em duality involution} 
$\check{H} \rightarrow \check{H}$ defined in \S \ref{dualityinvolution},
for which we don't know a reference. (This  assertion has content
 even in abelian Satake if we work over coefficient field $\kk=\Q$.)



The statement about Poisson structure 
(\S\ref{Poisson local conj} but even the stronger statement discussed in \S \ref{Poisson from loop}) was also proven by Bezrukavnikov and Finkelberg \cite{BezFink}. 
Finally, the 
statement about Galois actions does not apparently
appear in the literature, but
we have sketched a proof after \S \ref{Satake thm-arithmetic};
see also ~\cite{xinwenSatake}, 
~\cite{richarzscholbachmotivic}, and ~\cite{romaICM}.


 
 

 
  
  




 



 





\subsubsection{The trivial period}
We now take $X$ to be the point.
Thus $\Sph_X$ is simply the category of constructible sheaves on $BG$. That is to say (see \cite{BL}), 
  taking into account the formality of the cohomology of $BG$, 
$\Sph_X$ is simply the category of perfect modules under $H^*(BG)$. 
 
 
 In this case, $\Mv$ is the Whittaker model, that is to say,
 the Hamiltonian $\Gv$-space obtained by Whittaker indcution
 of the point under the principal $\SL_2 \rightarrow \Gv$;
 and 
 $\Mv/\Gv\simeq \fc_G$ is the Kostant slice.
 The equivalence as abstract categories follows from the identification of the equivariant cohomology ring $H^*(BG)$ with the shear of the ring of invariant polynomials $\cO(\fgxv)^{\Gv}$. The equivalence as module categories for the Hecke category is a theorem of Bezrukavnikov-Finkelberg~\cite{BezFink}  (the same paper also proves the compatibility of the Poisson bracket with loop rotation equivariance). 




\subsubsection{The Whittaker period} \label{sssWhittaker}
Dually, we consider the Whittaker model on the automorphic side. In other words, we take $M=T^\ast G\GIT_\psi U$. In this case the Hecke category $\Sph_M$ is the category $\Shv(G_F/G_O)^{U(F),\psi}$ of Whittaker sheaves on the Grassmannian. The dual period is $\Mv=pt$, so that $\QCshear(\Mv/\Gv)\simeq Rep(\Gv)^{\shear}.$ The resulting equivalence of categories is due to Frenkel-Gaitsgory-Vilonen~\cite{FGV} (see also~\cite{ABBGM}).

\subsubsection{Other examples} \label{OtherExamples}
Several other instances of the local conjecture have been proved recently --  verifying at least
the ``Hecke'' desideratum of the statement, although it is likely that the proofs give more. 
  
Hilburn and Raskin \cite{HilburnRaskin} prove a fully ramified, de Rham version of the local conjecture for the Iwasawa--Tate period.

 Braverman, Dhillon, Finkelberg, Raskin and Travkin \cite{RaskinNisyros}, and Teleman \cite{telemancoulomb} discuss geometric counterparts to the Weil representation and the construction of Coulomb branches (hence formulation of the local conjecture) in unpolarized settings.
 

Chen, Macerato, Nadler, and O'Brien \cite{CMNO} prove the local conjecture in the case $X = GL_{2n}/ Sp_{2n}$ and $\Mv=T^*(GL_{2n}/GL_n \ltimes U, \psi)\simeq GL_{2n}\times^{GL_n} M_n$
(in automorphic terminology, the ``symplectic period'' studied by Jacquet and Rallis \cite{JRsymplectic}). 

 Chen and Nadler \cite{ChenNadler} construct an equivalence, in the case of $X$ a symmetric variety, between the category  $\Hecke^X$ and a  category of sheaves
 arising in global {\em real} Langlands: sheaves on the space of principal bundles for a certain real form of $G$ over the real projective line. They show, among other results,
 the formality of the category $\mathcal{H}^X$ in this case, see \cite[Theorem 13.4]{ChenNadler}. 

The results of Macerato and Taylor \cite{MT} (when combined with \cite{ChenNadler}) imply that the local category for the symmetric variety $X=PSL_2/PO_2$ (which is outside of our hyperspherical setting due to the presence of Type N roots) contains a block equivalent to representations of quantum $SL_2$ at a fourth root of unity. This suggests that in this generality one should expect interesting braided ($E_2$) tensor categories to appear instead of the symmetric ones in our conjecture.  

   
Devalapurkar \cite{Devalapurkar}  proves  the local conjecture for the case of homogeneous affine spherical varieties of rank $1$,   modulo
certain hypotheses relating to placidity and evenness.
Moreover, in \cite{sanathtriple}, under the same hypotheses, he proves the local conjecture in the case of the triple product $L$-function 
(the diagonal inclusion of $\PGL_2$ into $\PGL_2^{\times 3}$).


The papers~\cite{BravermanMirabolic} and ~\cite{BravermanOrthosymplectic} of Braverman, Finkelberg, Ginzburg and Travkin prove the local conjecture (in a Koszul dual formulation)
in cases corresponding to:
\begin{itemize}
\item[-] $X = \GL_n$ as $G = \GL_n \times \GL_{n-1}$-space,  
\item[-] $X=\GL_n\times \AA^n$ as $G = \GL_n \times \GL_n$-space
 \item[-] $X=\SO_n$ as $G =\SO_n \times \SO_{n-1}$-space.
\end{itemize}
 In automorphic terminology, these correspond to the Rankin--Selberg
periods for $\GL_n \times \GL_{n-1}$ and $\GL_n\times \GL_n$ ~\cite{JPSRS} and the Gross--Prasad period for $\SO_n \times \SO_{n-1}$.  Travkin and Yang \cite{TravkinYangI} prove
the local conjecture  in the case of the 
the Rankin-Selberg period for $\GL_m \times \GL_n$ when $m < n-1$; the dual is then
  $\Xv=\mathrm{Mat}_{m\times n}$ acted on by $\Gv=\GL_m\times \GL_n$.

\begin{remark}[The Gaiotto Conjecture] \index{quantum geometric Langlands}
The geometric Langlands correspondence, at least in de Rham and Betti forms, has a so-called {\em quantum} deformation introduced by Feigin, Frenkel and Stoyanovsky, in which the automorphic categories are replaced by categories of twisted sheaves on moduli of $G$-bundles, see~\cite{gaitsgoryquantum, FrenkelGaiotto,BettiLanglands} and references therein. The spectral side has a description, in the Betti version, in terms of categories of representations of quantum groups. It is a natural question which forms of the relative Langlands conjectures admit quantum deformations -- it is easy to see that many periods do not admit such deformations, and even in cases that do (such as the group case) the deformed local category becomes much smaller or trivial. The Gaiotto conjecture provides a quantum deformation of the local conjecture for a family of periods where (like the Whittaker case) the deformed category is of the same size. Remarkably, these cases correspond to quantum supergroups, with $\Gv$ as the even part and $\Mv$ as the odd part, and include all the Rankin-Selberg and Gross-Prasad type integrals in the previous paragraph. 

The Gaiotto conjecture is formulated in~\cite[\S 2]{BravermanMirabolic}, and the quantum analogs of the above cases have now been proven for generic level in~\cite{BravermanOrthosymplecticII},~\cite{TravkinYangI} and ~\cite{TravkinYangII} (the Whittaker case corresponds to the {\em Fundamental Local Equivalence}, proven for irrational level in~\cite{GaitsgoryFLE} and for rational level in~\cite{rationalFLE}). Crucially, these conjectural descriptions are equivalences of {\em monoidal} categories, with the monoidal structure coming from factorization corresponding to the braided tensor product coming from quantum groups. 
 It would be very interesting to compare these spectral models with ours, and to apply the techniques developed in these papers to construct monoidal (or even braided monoidal) structures on the categories $\Hecke^X$ in general, see \S ~\ref{factorizable Hecke} and Problem ~\ref{localconstancyHeckeX}.
 \end{remark}
 
 
 

